STDG: Semi-Teacher-Student Training Paradigram for Depth-guided One-stage Scene Graph Generation

Scene Graph Generation is a critical enabler of environmental comprehension for autonomous robotic systems. Most of existing methods, however, are often thwarted by the intricate dynamics of background complexity, which limits their ability to fully decode the inherent topological information of the environment. Additionally, the wealth of contextual information encapsulated within depth cues is often left untapped, rendering existing approaches less effective. To address these shortcomings, we present STDG, an avant-garde Depth-Guided One-Stage Scene Graph Generation methodology. The innovative architecture of STDG is a triad of custom-built modules: The Depth Guided HHA Representation Generation Module, the Depth Guided Semi-Teaching Network Learning Module, and the Depth Guided Scene Graph Generation Module. This trifecta of modules synergistically harnesses depth information, covering all aspects from depth signal generation and depth feature utilization, to the final scene graph prediction. Importantly, this is achieved without imposing additional computational burden during the inference phase. Experimental results confirm that our method significantly enhances the performance of one-stage scene graph generation baselines.

==> first_pic.tex <==
 \begin{figure*} %H为当前位置，!htb为忽略美学标准，htbp为浮动图形
    \centering %图片居中
    \includegraphics[width=1.0\textwidth]{image/model.pdf} %插入图片，[]中设置图片大小，{}中是图片文件名
    \caption{Structure of Depth guided semi-supervised one-stage scene graph generation model. The depth model would be trained at first. Then it would be used as an teacher to teach the rgb model to learn how to focus on certain object.} %最终文档中希望显示的图片标题
    \label{Fig.Model} %用于文内引用的标签
    \end{figure*}
